A Sinkhorn Regularized Adversarial Network for Image Guided DEM Super-resolution using Frequency Selective Hybrid Graph Transformer

Digital Elevation Model (DEM) is an essential aspect in the remote sensing (RS) domain to analyze various applications related to surface elevations. Here, we address the generation of high-resolution (HR) DEMs using HR multi-spectral (MX) satellite imagery as a guide by introducing a novel hybrid transformer model consisting of Densely connected Multi-Residual Block (DMRB) and multi-headed Frequency Selective Graph Attention (M-FSGA). To promptly regulate this process, we utilize the notion of discriminator spatial maps as the conditional attention to the MX guide. Further, we present a novel adversarial objective related to optimizing Sinkhorn distance with classical GAN. In this regard, we provide both theoretical and empirical substantiation of better performance in terms of vanishing gradient issues and numerical convergence. Based on our experiments on 4 different DEM datasets, we demonstrate both qualitative and quantitative comparisons with available baseline methods and show that the performance of our proposed model is superior to others with sharper details and minimal errors.

==> Tables/Ablation3.tex <==
\begin{table}[tb]
\centering
\begin{minipage}[b]{.3\textwidth}
\centering
\caption{Abalation study for different patch sizes in FSGT}
\label{tab:patch}
\resizebox{0.675\textwidth}{!}{%
\begin{tabular}{c|cc}
\hline
\textbf{Patch Size} & \textbf{PSNR}  & \textbf{SSIM}  \\ \hline
$3\times 3$                   & 34.81          & 90.08          \\
$5\times 5$                   & 34.92          & 90.23          \\
$7\times 7$                  & \textbf{35.06} & \textbf{90.49} \\
$9\times 9$                  & 34.84          & 90.15          \\
$11\times 11$                  & 34.74          & 89.79          \\ \hline
\end{tabular}%
}
\end{minipage}
\quad
\begin{minipage}[b]{.3\textwidth}
\centering
\caption{Ablation study for different numbers of heads ($M$) in M-FSGA}
\label{tab:heads}
\resizebox{0.8\textwidth}{!}{%
\begin{tabular}{c|ccc}
\hline
\textbf{\begin{tabular}[c]{@{}c@{}}Number\\ of heads\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Params\\ (M)\end{tabular}} & \textbf{PSNR} & \textbf{SSIM} \\ \hline
4                        & 7.41                & 34.55         & 89.36         \\
8                        & 11.08               & 34.82         & 89.85         \\
12                       & 16.37               & 34.94         & 90.15         \\
16                       & 21.36               & 35.06         & 90.49         \\
24                       & 30.22               & 35.07         & 90.33         \\ \hline
\end{tabular}%
}
\end{minipage}
\quad
\begin{minipage}[b]{.3\textwidth}
\centering
\caption{Model size comparison ($\times4$ SR). Output size is $512\times 512 \times 3$}
\label{tab:computation}
\resizebox{\textwidth}{!}{%
\begin{tabular}{c|cccc}
\hline
\textbf{Model} & \textbf{\begin{tabular}[c]{@{}c@{}}Params\\ (M)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}FLOPs\\ (G)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Runtime\\ (ms)\end{tabular}} & \textbf{PSNR} \\ \hline
SwinIR \cite{swin}        & 11.90               & 215.3              & 152.2                 & 34.91         \\
CAT \cite{cat}            & 16.60               & 360.7              & 351.8                 & 34.96         \\
HAN \cite{han}            & 16.07               & 269.1              & 245.7                 & 34.94         \\
ART \cite{art}            & 11.87               & 278.3              & 261.3                 & 35.02         \\
FSGT (ours)    & 21.36               & 189.4              & 149.6                 & 35.06         \\ \hline
\end{tabular}%
}
\end{minipage}
\vspace{-0.4cm}
\end{table}

==> Tables/Ablation3_V2.tex <==
\begin{table}[tb]
\centering
\begin{minipage}[b]{.3\textwidth}
\centering
\caption{Abalation study for different patch sizes in FSGT}
\label{tab:patch}
\resizebox{0.675\textwidth}{!}{%
\begin{tabular}{c|cc}
\hline
\textbf{Patch Size} & \textbf{PSNR}  & \textbf{SSIM}  \\ \hline
$3\times 3$                   & 33.81          & 89.08          \\
$5\times 5$                   & 33.92          & 89.23          \\
$7\times 7$                  & \textbf{34.55} & \textbf{89.49} \\
$9\times 9$                  & 34.34          & 89.15          \\
$11\times 11$                  & 34.28          & 89.09          \\ \hline
\end{tabular}%
}
\end{minipage}
\quad
\begin{minipage}[b]{.3\textwidth}
\centering
\caption{Ablation study for different numbers of heads ($M$) in M-FSGA}
\label{tab:heads}
\resizebox{0.8\textwidth}{!}{%
\begin{tabular}{c|ccc}
\hline
\textbf{\begin{tabular}[c]{@{}c@{}}Number\\ of heads\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Params\\ (M)\end{tabular}} & \textbf{PSNR} & \textbf{SSIM} \\ \hline
4                        & 5.29                & 34.34         & 89.04         \\
8                        & 7.41               & 34.55         & 89.36         \\
12                       & 16.37               & 34.59         & 89.64         \\
16                       & 21.36               & 34.61         & 90.09         \\
24                       & 30.22               & 34.72         & 90.13         \\ \hline
\end{tabular}%
}
\end{minipage}
\quad
\begin{minipage}[b]{.3\textwidth}
\centering
\caption{Model size comparison ($\times4$ SR). Output size is $512\times 512 \times 3$}
\label{tab:computation}
\resizebox{\textwidth}{!}{%
\begin{tabular}{c|cccc}
\hline
\textbf{Model} & \textbf{\begin{tabular}[c]{@{}c@{}}Params\\ (M)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}FLOPs\\ (G)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Runtime\\ (ms)\end{tabular}} & \textbf{PSNR} \\ \hline
SwinIR \cite{swin}        & 11.90               & 215.3              & 152.2                 & 34.41         \\
CAT \cite{cat}            & 16.60               & 360.7              & 351.8                 & 34.16         \\
HAN \cite{han}            & 16.07               & 269.1              & 245.7                 & 33.94         \\
ART \cite{art}            & 11.87               & 278.3              & 261.3                 & 34.25         \\
FSGT (ours)    & 21.36               & 189.4              & 149.6                 & 34.55         \\ \hline
\end{tabular}%
}
\end{minipage}
\vspace{-0.4cm}
\end{table}
